Practical considerations for variable screening in the super learner

Estimating a prediction function is a fundamental component of many data analyses. The super learner ensemble, a particular implementation of stacking, has desirable theoretical properties and has been used successfully in many applications. Dimension reduction can be accomplished by using variable screening algorithms (screeners), including the lasso, within the ensemble prior to fitting other prediction algorithms. However, the performance of a super learner using the lasso for dimension reduction has not been fully explored in cases where the lasso is known to perform poorly. We provide empirical results that suggest that a diverse set of candidate screeners should be used to protect against poor performance of any one screener, similar to the guidance for choosing a library of prediction algorithms for the super learner. These results are further illustrated through the analysis of HIV-1 antibody data.

==> plots/pred-perf_gaussian_strong_matched.tex <==
\begingroup\fontsize{10}{12}\selectfont

\begin{longtable}[t]{r>{\raggedright\arraybackslash}p{5em}>{\raggedright\arraybackslash}p{5em}>{\raggedright\arraybackslash}p{5em}>{\raggedright\arraybackslash}p{5em}>{\raggedright\arraybackslash}p{5em}>{\raggedright\arraybackslash}p{5em}>{\raggedleft\arraybackslash}p{5em}>{\raggedleft\arraybackslash}p{5em}}
\caption{\label{tab:pred_perf_gaussian_strong_matched}Cross-validated R-squared for all candidate learners  in the super learner ensemble  (and the cSL and dSL for p = 2000).  Outcome type: continuous, relationship: strong.}\\
\toprule
n & p & Outcome relationship & Feature correlation & Candidate Learners & Candidate Screeners & Learner & Prediction performance & Optimal prediction performance\\
\midrule
\endfirsthead
\caption[]{Estimates of cross-validated prediction performance for all screener-learner pairs within the super learner. \textit{(continued)}}\\
\toprule
n & p & Outcome relationship & Feature correlation & Candidate Learners & Candidate Screeners & Learner & Prediction performance & Optimal prediction performance\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
500 & 2000 & Nonlinear & Uncorrelated & All & All & dSL & 0.634 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All & All (+none) & dSL & 0.736 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All & All (-lasso) & dSL & 0.634 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All & Lasso & dSL & 0.513 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All & None & dSL & 0.737 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & All & dSL & 0.634 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & All (+none) & dSL & 0.736 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & All (-lasso) & dSL & 0.634 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & Lasso & dSL & 0.513 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & None & dSL & 0.737 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All & None & Lasso & 0.585 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All & All & cSL & 0.673 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All & All (+none) & cSL & 0.744 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All & All (-lasso) & cSL & 0.673 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All & Lasso & cSL & 0.559 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All & None & cSL & 0.739 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & All & cSL & 0.673 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & All (+none) & cSL & 0.744 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & All (-lasso) & cSL & 0.673 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & Lasso & cSL & 0.559 & 0.856\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & None & cSL & 0.715 & 0.856\\
500 & 2000 & Nonlinear & Correlated & All & All & dSL & 0.678 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All & All (+none) & dSL & 0.678 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All & All (-lasso) & dSL & 0.678 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All & Lasso & dSL & 0.223 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All & None & dSL & 0.548 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All (-lasso) & All & dSL & 0.678 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All (-lasso) & All (+none) & dSL & 0.678 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All (-lasso) & All (-lasso) & dSL & 0.678 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All (-lasso) & Lasso & dSL & 0.223 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All (-lasso) & None & dSL & 0.548 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All & None & Lasso & 0.010 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All & All & cSL & 0.688 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All & All (+none) & cSL & 0.565 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All & All (-lasso) & cSL & 0.689 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All & Lasso & cSL & 0.264 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All & None & cSL & 0.246 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All (-lasso) & All & cSL & 0.688 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All (-lasso) & All (+none) & cSL & 0.565 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All (-lasso) & All (-lasso) & cSL & 0.689 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All (-lasso) & Lasso & cSL & 0.264 & 0.758\\
500 & 2000 & Nonlinear & Correlated & All (-lasso) & None & cSL & 0.246 & 0.758\\
500 & 2000 & Linear & Uncorrelated & All & All & dSL & 0.913 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All & All (+none) & dSL & 0.924 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All & All (-lasso) & dSL & 0.911 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All & Lasso & dSL & 0.907 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All & None & dSL & 0.924 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & All & dSL & 0.913 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & All (+none) & dSL & 0.913 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & All (-lasso) & dSL & 0.911 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & Lasso & dSL & 0.907 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & None & dSL & 0.892 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All & None & Lasso & 0.924 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All & All & cSL & 0.895 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All & All (+none) & cSL & 0.887 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All & All (-lasso) & cSL & 0.890 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All & Lasso & cSL & 0.913 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All & None & cSL & 0.922 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & All & cSL & 0.895 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & All (+none) & cSL & 0.898 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & All (-lasso) & cSL & 0.890 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & Lasso & cSL & 0.913 & 0.932\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & None & cSL & 0.876 & 0.932\\
500 & 2000 & Linear & Correlated & All & All & dSL & 0.950 & 0.951\\
500 & 2000 & Linear & Correlated & All & All (+none) & dSL & 0.950 & 0.951\\
500 & 2000 & Linear & Correlated & All & All (-lasso) & dSL & 0.950 & 0.951\\
500 & 2000 & Linear & Correlated & All & Lasso & dSL & 0.933 & 0.951\\
500 & 2000 & Linear & Correlated & All & None & dSL & 0.941 & 0.951\\
500 & 2000 & Linear & Correlated & All (-lasso) & All & dSL & 0.950 & 0.951\\
500 & 2000 & Linear & Correlated & All (-lasso) & All (+none) & dSL & 0.950 & 0.951\\
500 & 2000 & Linear & Correlated & All (-lasso) & All (-lasso) & dSL & 0.950 & 0.951\\
500 & 2000 & Linear & Correlated & All (-lasso) & Lasso & dSL & 0.933 & 0.951\\
500 & 2000 & Linear & Correlated & All (-lasso) & None & dSL & 0.919 & 0.951\\
500 & 2000 & Linear & Correlated & All & None & Lasso & 0.941 & 0.951\\
500 & 2000 & Linear & Correlated & All & All & cSL & 0.439 & 0.951\\
500 & 2000 & Linear & Correlated & All & All (+none) & cSL & 0.926 & 0.951\\
500 & 2000 & Linear & Correlated & All & All (-lasso) & cSL & 0.438 & 0.951\\
500 & 2000 & Linear & Correlated & All & Lasso & cSL & 0.935 & 0.951\\
500 & 2000 & Linear & Correlated & All & None & cSL & 0.929 & 0.951\\
500 & 2000 & Linear & Correlated & All (-lasso) & All & cSL & 0.439 & 0.951\\
500 & 2000 & Linear & Correlated & All (-lasso) & All (+none) & cSL & 0.926 & 0.951\\
500 & 2000 & Linear & Correlated & All (-lasso) & All (-lasso) & cSL & 0.438 & 0.951\\
500 & 2000 & Linear & Correlated & All (-lasso) & Lasso & cSL & 0.935 & 0.951\\
500 & 2000 & Linear & Correlated & All (-lasso) & None & cSL & 0.877 & 0.951\\*
\end{longtable}
\endgroup{}


==> plots/pred-perf_gaussian_weak_matched.tex <==
\begingroup\fontsize{10}{12}\selectfont

\begin{longtable}[t]{r>{\raggedright\arraybackslash}p{5em}>{\raggedright\arraybackslash}p{5em}>{\raggedright\arraybackslash}p{5em}>{\raggedright\arraybackslash}p{5em}>{\raggedright\arraybackslash}p{5em}>{\raggedright\arraybackslash}p{5em}>{\raggedleft\arraybackslash}p{5em}>{\raggedleft\arraybackslash}p{5em}}
\caption{\label{tab:pred_perf_gaussian_weak_matched}Cross-validated R-squared for all candidate learners  in the super learner ensemble  (and the cSL and dSL for p = 2000).  Outcome type: continuous, relationship: weak.}\\
\toprule
n & p & Outcome relationship & Feature correlation & Candidate Learners & Candidate Screeners & Learner & Prediction performance & Optimal prediction performance\\
\midrule
\endfirsthead
\caption[]{Estimates of cross-validated prediction performance for all screener-learner pairs within the super learner. \textit{(continued)}}\\
\toprule
n & p & Outcome relationship & Feature correlation & Candidate Learners & Candidate Screeners & Learner & Prediction performance & Optimal prediction performance\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
500 & 2000 & Nonlinear & Uncorrelated & All & All & dSL & 0.300 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All & All (+none) & dSL & 0.331 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All & All (-lasso) & dSL & 0.300 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All & Lasso & dSL & 0.250 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All & None & dSL & 0.324 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & All & dSL & 0.300 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & All (+none) & dSL & 0.303 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & All (-lasso) & dSL & 0.300 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & Lasso & dSL & 0.250 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & None & dSL & 0.091 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All & None & Lasso & 0.315 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All & All & cSL & 0.001 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All & All (+none) & cSL & 0.061 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All & All (-lasso) & cSL & 0.044 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All & Lasso & cSL & 0.263 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All & None & cSL & 0.327 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & All & cSL & 0.001 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & All (+none) & cSL & -0.007 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & All (-lasso) & cSL & 0.044 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & Lasso & cSL & 0.263 & 0.667\\
500 & 2000 & Nonlinear & Uncorrelated & All (-lasso) & None & cSL & 0.184 & 0.667\\
500 & 2000 & Nonlinear & Correlated & All & All & dSL & 0.681 & 0.744\\
500 & 2000 & Nonlinear & Correlated & All & All (+none) & dSL & 0.681 & 0.744\\
500 & 2000 & Nonlinear & Correlated & All & All (-lasso) & dSL & 0.681 & 0.744\\
500 & 2000 & Nonlinear & Correlated & All & Lasso & dSL & 0.601 & 0.744\\
500 & 2000 & Nonlinear & Correlated & All & None & dSL & 0.559 & 0.744\\
500 & 2000 & Nonlinear & Correlated & All (-lasso) & All & dSL & 0.681 & 0.744\\
500 & 2000 & Nonlinear & Correlated & All (-lasso) & All (+none) & dSL & 0.681 & 0.744\\
500 & 2000 & Nonlinear & Correlated & All (-lasso) & All (-lasso) & dSL & 0.681 & 0.744\\
500 & 2000 & Nonlinear & Correlated & All (-lasso) & Lasso & dSL & 0.601 & 0.744\\
500 & 2000 & Nonlinear & Correlated & All (-lasso) & None & dSL & 0.559 & 0.744\\
500 & 2000 & Nonlinear & Correlated & All & None & Lasso & 0.226 & 0.744\\
500 & 2000 & Nonlinear & Correlated & All & All & cSL & 0.257 & 0.744\\
500 & 2000 & Nonlinear & Correlated & All & All (+none) & cSL & 0.409 & 0.744\\
500 & 2000 & Nonlinear & Correlated & All & All (-lasso) & cSL & 0.078 & 0.744\\
500 & 2000 & Nonlinear & Correlated & All & Lasso & cSL & 0.621 & 0.744\\
500 & 2000 & Nonlinear & Correlated & All (-lasso) & All & cSL & 0.257 & 0.744\\
500 & 2000 & Nonlinear & Correlated & All (-lasso) & All (+none) & cSL & 0.409 & 0.744\\
500 & 2000 & Nonlinear & Correlated & All (-lasso) & All (-lasso) & cSL & 0.078 & 0.744\\
500 & 2000 & Nonlinear & Correlated & All (-lasso) & Lasso & cSL & 0.621 & 0.744\\
500 & 2000 & Linear & Uncorrelated & All & All & dSL & 0.646 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All & All (+none) & dSL & 0.648 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All & All (-lasso) & dSL & 0.646 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All & Lasso & dSL & 0.599 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All & None & dSL & 0.651 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & All & dSL & 0.646 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & All (+none) & dSL & 0.646 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & All (-lasso) & dSL & 0.646 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & Lasso & dSL & 0.599 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & None & dSL & 0.450 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All & None & Lasso & 0.651 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All & All & cSL & 0.604 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All & All (+none) & cSL & 0.557 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All & All (-lasso) & cSL & 0.604 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All & Lasso & cSL & 0.610 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All & None & cSL & 0.595 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & All & cSL & 0.604 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & All (+none) & cSL & 0.554 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & All (-lasso) & cSL & 0.604 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & Lasso & cSL & 0.610 & 0.667\\
500 & 2000 & Linear & Uncorrelated & All (-lasso) & None & cSL & 0.464 & 0.667\\
500 & 2000 & Linear & Correlated & All & All & dSL & 0.785 & 0.796\\
500 & 2000 & Linear & Correlated & All & All (+none) & dSL & 0.786 & 0.796\\
500 & 2000 & Linear & Correlated & All & All (-lasso) & dSL & 0.785 & 0.796\\
500 & 2000 & Linear & Correlated & All & Lasso & dSL & 0.762 & 0.796\\
500 & 2000 & Linear & Correlated & All & None & dSL & 0.788 & 0.796\\
500 & 2000 & Linear & Correlated & All (-lasso) & All & dSL & 0.785 & 0.796\\
500 & 2000 & Linear & Correlated & All (-lasso) & All (+none) & dSL & 0.785 & 0.796\\
500 & 2000 & Linear & Correlated & All (-lasso) & All (-lasso) & dSL & 0.785 & 0.796\\
500 & 2000 & Linear & Correlated & All (-lasso) & Lasso & dSL & 0.762 & 0.796\\
500 & 2000 & Linear & Correlated & All (-lasso) & None & dSL & 0.659 & 0.796\\
500 & 2000 & Linear & Correlated & All & None & Lasso & 0.788 & 0.796\\
500 & 2000 & Linear & Correlated & All & All & cSL & 0.772 & 0.796\\
500 & 2000 & Linear & Correlated & All & All (+none) & cSL & 0.738 & 0.796\\
500 & 2000 & Linear & Correlated & All & All (-lasso) & cSL & 0.773 & 0.796\\
500 & 2000 & Linear & Correlated & All & Lasso & cSL & 0.770 & 0.796\\
500 & 2000 & Linear & Correlated & All & None & cSL & 0.734 & 0.796\\
500 & 2000 & Linear & Correlated & All (-lasso) & All & cSL & 0.772 & 0.796\\
500 & 2000 & Linear & Correlated & All (-lasso) & All (+none) & cSL & 0.737 & 0.796\\
500 & 2000 & Linear & Correlated & All (-lasso) & All (-lasso) & cSL & 0.773 & 0.796\\
500 & 2000 & Linear & Correlated & All (-lasso) & Lasso & cSL & 0.770 & 0.796\\
500 & 2000 & Linear & Correlated & All (-lasso) & None & cSL & 0.556 & 0.796\\*
\end{longtable}
\endgroup{}

